Robust Persistence Diagrams using Reproducing Kernels

Persistent homology has become an important tool for extracting geometric and topological features from data, whose multi-scale features are summarized in a persistence diagram. From a statistical perspective, however, persistence diagrams are very sensitive to perturbations in the input space. In this work, we develop a framework for constructing robust persistence diagrams from superlevel filtrations of robust density estimators constructed using reproducing kernels. Using an analogue of the influence function on the space of persistence diagrams, we establish the proposed framework to be less sensitive to outliers. The robust persistence diagrams are shown to be consistent estimators in bottleneck distance, with the convergence rate controlled by the smoothness of the kernel. This, in turn, allows us to construct uniform confidence bands in the space of persistence diagrams. Finally, we demonstrate the superiority of the proposed approach on benchmark datasets.

==> sections/simulations.tex <==
%%%%%% Section 1: Introduction  %%%%%%%%%%%%%%%%%%%%%%%%
\section{Simulations and Data Analysis}
\label{simulations}

\subsection{Bottleneck Distances}
\label{sim-bottleneck}

Let $\pr$ be the distribution associated with a true signal supported on a manifold of interest, $\M$, and let $\qr$ be the distribution associated with some isosyncratic noise supported on the ambient space. For $\pi \in (0,1)$, suppose the observed data $\Xn$ comes from the distribution $\pt = (1-\pi)\pr + \pi\qr$. The objective in this simulation is to determine how close $\dgm{\fs}$ is to the noiseless version $\dgm{f}$, as opposed to $\dgm{\fsbar}$.

In this case, let $\M = \mathbb{S}_1 \cup \mathbb{S}_2$, where $\mathbb{S}_1$ and $\mathbb{S}_2$ are circles contained inside the square $\X = [-4,4]^2$. The signal and noise are given by $\pr \sim Unif(\M)$ and $\qr \sim Unif(\X)$ and the mixture component $\pi = 0.3$. Let $\Xn$ be observed from $\pt$, and $\Yn$ be observed from $\pr$.

Additionally, for the sake of simplicity in this section, the Robust KDE associated with $\Xn$ is denoted by $f^n_{\pt}$, the KDE associated with $\Xn$ by $\bar{f}^n_{\pt}$ and the KDE from the noiseless version $\Yn$ by $\bar{f}^n_{\pr}$. The bottleneck distance between persistence diagrams is denoted by $\Winf(D_1,D_2)$ for every pair of diagrams $D_1,D_2$.

Instead, for $N=500$ runs, we simulate $N$ different point-clouds $X_n^{(1)},X_n^{(2)},\dots,X_n^{(N)}$ from $\pt$ (similarly for $\Yn$). Figure \ref{fig:bottleneck} (a) shows one such realization. For each run, we also compute the two bottleneck distances
\eq{
\Winf^{(j)}\pa{\dgm{(f^n_{\pt})},\dgm{(\bar{f}^n_{\pr})}} \ \  \text{ and} \ \ \Winf^{(j)}\pa{\dgm{(\bar{f}^n_{\pt})},\dgm{(\bar{f}^n_{\pr}})} \ \ \text{for } j = 1, 2, \dots, N\nn
}

Figure \ref{fig:bottleneck} (b) shows the boxplot for the two bottleneck distances. The figure shows that the RKDE constructed on the noisy sample is indeed closer (topologically) to the KDE on the noiseless sample, as opposed to the the KDE on the noisy sample.

\begin{figure}
  \centering
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{./plots/bottleneck/cloud.pdf}
    \caption{Point cloud for a realization of $\Xn$ when $\pi = 10\%$}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{./plots/bottleneck-new/boxplot-sim1.pdf}
    \caption{Corresponding boxplot for bottleneck distances}
  \end{subfigure}
  \caption{Comparison of $\Winf\pa{\dgm{(f^n_{\pt})},\dgm{(\bar{f}^n_{\pr})}}$ with $\Winf\pa{\dgm{(\bar{f}^n_{\pt})},\dgm{(\bar{f}^n_{\pr}})}$}
  \label{fig:bottleneck}
\end{figure}



\begin{figure}
  \centering
  % \begin{subfigure}[b]{0.3\linewidth}
  %   \includegraphics[width=\linewidth]{./plots/bottleneck-new/boxplot-sim1.pdf}
  %   \caption{$\pi=10\%$}
  % \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{./plots/bottleneck-new/boxplot-sim2.pdf}
    \caption{$\pi=20\%$}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{./plots/bottleneck-new/boxplot-sim3.pdf}
    \caption{$\pi=30\%$}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{./plots/bottleneck-new/boxplot-sim4.pdf}
    \caption{$\pi=40\%$}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{./plots/bottleneck-new/boxplot-sim5.pdf}
    \caption{$\pi=50\%$}
  \end{subfigure}
  \caption{Bottleneck Distance Simulation}
  \label{fig-bottleneck-noises}
\end{figure}

\begin{figure}
  \centering
  % \begin{subfigure}[b]{0.3\linewidth}
  %   \includegraphics[width=\linewidth]{./plots/bottleneck-new/scatterplot-sim1.pdf}
  %   \caption{$\pi=10\%$}
  % \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{./plots/bottleneck-new/scatterplot-sim2.pdf}
    \caption{$\pi=20\%$}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{./plots/bottleneck-new/scatterplot-sim3.pdf}
    \caption{$\pi=30\%$}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{./plots/bottleneck-new/scatterplot-sim4.pdf}
    \caption{$\pi=40\%$}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{./plots/bottleneck-new/scatterplot-sim5.pdf}
    \caption{$\pi=50\%$}
  \end{subfigure}
  \caption{Bottleneck Distance Simulation}
  \label{fig-scatterplot-noises}
\end{figure}

% \begin{figure}[H]
%   \includegraphics[width=0.9\linewidth]{./plots/bottleneck/cloud.pdf}
%   % \caption{Test}
%   \label{fig1}
% \end{figure}
%
% \begin{figure}[H]
%   \includegraphics[width=0.9\linewidth]{./plots/bottleneck/boxplot.pdf}
%   % \caption{Test}
%   \label{fig1}
% \end{figure}




\subsection{Random Circles}
\label{sim-circles}

In this simulation study, we generate random circles $\mathbb{S}_1, \mathbb{S}_2,\dots,\mathbb{S}_{\mathbf{N}}$ with centers in a unit square -- the number of such circles, $\mathbf{N}$, is a Poisson random variable. For each realization, the signal is a distribution $\pr \sim Unif(\bigcup^\mathbf{N}_{i=1}{\mathbb{S}_i})$ and the noise $\qr$ is uniformly supported on the enclosing rectangle. $\Xn$ is sampled from the mixture distribution $\pt$. We generate $100$ such point-clouds for $N_1, N_2, \dots, N_{100} \sim \mathbf{N}$. Figure \ref{fig2} shows three examples of point-clouds. We

\begin{figure}[H]
  \includegraphics[width=1\linewidth]{./plots/circles/sample.pdf}
  \caption{Point-clouds for $\mathbf{N} = 0, 2, 5$}
  \label{fig2}
\end{figure}

The objective of this simulation is to use persistence diagrams from the sublevel filtrations to predict the number of circles in a given point-cloud. The empirical version of the distance-to-measure computes a weighted k-NN density estimate, where the nearest neighbour parameter $k$ is related to $m$ via the relationship $m = \f{k}{n}$. \citep{chazal2017robust}. Additionally, for the experiments on RKDE in \citep[Section 7.2]{kim2012robust}, the kernel bandwidth $\s$ is chosen as the the median distance of each $\xv_i \in \Xn$ to its $k^{th}$ nearest neighbour. In order to compare these estimators at similar resolutions, the three different choices for $m$ and $\s$ each correspond to $k = 5$, $k=7$ and $k=10$. For each $1 \le j \le 100$, we compute the persistence diagrams  $\dgm\pa{\fns}$, $\dgm\pa{\fnsbar}$ and $\dgm\pa{\delta^n_m}$ for three different choices of parameters for $\s$ and $m$ -- computing, in total, $3\times 3\times 100$ persistence diagrams.

\begin{figure}[H]
  \includegraphics[width=0.99\linewidth]{./plots/circles/dgms.pdf}
  \caption{$\dgm(\fns)$, $\dgm(\fnsbar)$ and $\dgm(\delta^n_m)$ for $\mathbf{N} = 4$ and $k=7$}
  \label{fig3}
\end{figure}


Figure \ref{fig3} shows an example of the three persistence diagrams when $N=4$ and $k=7$. For each persistence diagram $\dgm(f)$, we ``vectorize'' it by computing a $20\times 20$ persistence image $\Img(f)$ with bandwidth $h=0.015$ \citep{adams2017persistence}. This is shown in Figure \ref{fig4}

\begin{figure}[H]
  \includegraphics[width=0.99\linewidth]{./plots/circles/images.pdf}
  \caption{$\Img(\fns)$, $\Img(\fnsbar)$ and $\Img(\delta^n_m)$ for the Diagrams in Figure \ref{fig3}}
  \label{fig4}
\end{figure}

The persistence images are then split into a training and testing dataset (75:25 split) and are then trained using a linear support vector machine. The results based on averaging over 50 random splits for each $k$ are shown in Table \ref{tab1} below. Figure \ref{fig5} shows the mean squared prediction error as the bandwidth of the persistence image $h$ varies.

\begin{table}[ht]
\centering
\begin{tabular}{|c|rrr|}
  \hline
 & KDE & DTM & RKDE \\
 \hline
 \hline
  $k=5$ & 1.87 & 1.83 & 0.87 \\
  $k=7$ & 1.88 & 1.83 & 0.90 \\
  $k=10$ & 1.89 & 1.82 & 0.95 \\
   \hline
\end{tabular}
\caption{The average mean squared prediction error over 50 random splits}
\label{tab1}
\end{table}


\begin{figure}[H]
  \centering
  \begin{subfigure}[b]{0.32\linewidth}
    \includegraphics[width=\linewidth]{./plots/circles/k5/lines-42.pdf}
    \caption{$k=5$}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\linewidth}
    \includegraphics[width=\linewidth]{./plots/circles/k7/lines-42.pdf}
    \caption{$k=7$}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\linewidth}
    \includegraphics[width=\linewidth]{./plots/circles/k10/lines-42.pdf}
    \caption{$k=10$}
  \end{subfigure}

  \caption{The average mean squared prediction error as $h$ varies for different choices of $k$}
  \label{fig5}
\end{figure}





\subsection{mpeg7}
\label{sim-mpeg7}

For this simulation study, we examine how the RKDE, KDE and DTM fare in classifying some objects in the presence of noise. The data comes from the \texttt{mpeg7} dataset, which comprises of $1400$ images corresponding to $70$ different objects with $20$ images from each catergory.

% \begin{figure}[H]
%   \includegraphics[width=0.8\linewidth]{./plots/mpeg7/examples.pdf}
%   \caption{Examples of images from the \texttt{mpeg7} dataset}
%   \label{fig6}
% \end{figure}

We extract the boundary shape for each image by computing the image Laplacian for each object, and is considered as the true signal for the experiments. We sample the points for each image from the image-Laplacian and overlay it with some uniform ambient noise ($\pi = 0.5$). This is the observed point-cloud $\Xn$ for each image. This sampling procedure is shown in Figure \ref{fig7}.

We restrict our attention to three classes : \texttt{beetle}, \texttt{bone} and \texttt{spring}. For point-clouds from each class, we compute the persistence diagrams $\dgm(f)$ for $f \in \pb{\fns,\fnsbar,\delta^n_m}$, and ``vectorize'' them to $20\times 20$ persistence images as shown in Figure \ref{fig8}.

\begin{figure}[H]
  \includegraphics[width=0.9\linewidth]{./plots/mpeg7/conversion.pdf}
  \caption{Examples of images from the \texttt{mpeg7} dataset}
  \label{fig7}
\end{figure}


\begin{figure}[H]
  \includegraphics[width=0.9\linewidth]{./plots/mpeg7/3class.pdf}
  \caption{(Top) Examples from \texttt{beetle}, \texttt{bone} and \texttt{spring}. (Middle) The persistence diagrams $\dgm(\fns)$. (Bottom) Corresponding $20\times 20$ persistence images $\Img(\fns)$ with $h=0.02$}
  \label{fig8}
\end{figure}

The persistence images for the $0^{th}$ and $1^{st}$ homology are then concatenated for each point-cloud, and the data is split into separate training and testing datasets ($90$:$10$ split) and are then trained using a linear support vector machine. The results based on averaging over $100$ random splits are shown in the Table \ref{tab2} below. Figure \ref{fig9} plots the misclassification error as the bandwidth of the persistence image $h$ varies.

\begin{table}[ht]
\centering
\begin{tabular}{|c|c|}
  \hline
 & Misclassification Error \\
  \hline
  KDE & 17.16\% \\
  DTM & 23.33\% \\
  RKDE & 3.66\% \\
   \hline
\end{tabular}
\caption{The average misclassification error over 100 random splits}
\label{tab2}
\end{table}

\begin{figure}[H]
  \includegraphics[width=0.7\linewidth]{./plots/mpeg7/error-line.pdf}
  \caption{The average misclassification error over $100$ random splits as $h$ varies}
  \label{fig9}
\end{figure}

